From Lists to Emojis: How Format Bias Affects Model Alignment

In this paper, we study format biases in reinforcement learning from human feedback (RLHF). We observe that many widely-used preference models, including human evaluators, GPT-4, and top-ranking models on the RewardBench benchmark, exhibit strong biases towards specific format patterns, such as lists, links, bold text, and emojis. Furthermore, large language models (LLMs) can exploit these biases to achieve higher rankings on popular benchmarks like AlpacaEval and LMSYS Chatbot Arena. One notable example of this is verbosity bias, where current preference models favor longer responses that appear more comprehensive, even when their quality is equal to or lower than shorter, competing responses. However, format biases beyond verbosity remain largely underexplored in the literature. In this work, we extend the study of biases in preference learning beyond the commonly recognized length bias, offering a comprehensive analysis of a wider range of format biases. Additionally, we show that with a small amount of biased data (less than 1%), we can inject significant bias into the reward model. Moreover, these format biases can also be easily exploited by downstream alignment algorithms, such as best-of-n sampling and online iterative DPO, as it is usually easier to manipulate the format than to improve the quality of responses. Our findings emphasize the need to disentangle format and content both for designing alignment algorithms and evaluating models.

==> tables/emoji-example.tex <==
\begin{figure*}[htp]
\centering
\begin{promptbox}[Emoji Example]{lightgreen}
\noindent \textbf{Instruction:} Write a good Twitter Bio. Try to cover all the provided main points in your generated bio.\\

Name: Jane

Main points:

- Architect

- Interested in Tech

Written in first person

Use casual tone

\begin{multicols}{2}
    % Green dashed box with darker green border
    \begin{simpledashbox}{green}{green!70!black}
    \vspace{-0.1cm}
    \noindent \textbf{GPT4-1106-preview ({\color{green}\textbf{Preferred}}):} \\
    Architect by day, tech enthusiast by night 
    \includegraphics[height=1em]{latex/figs/emoji.png}. 
    I'm Jane, living my life one blueprint and gadget at a time. Crafting spaces, exploring innovation. Let's build and geek out together! \#ArchitectureLover \#TechWhiz
    \end{simpledashbox}

    \columnbreak

    % Red dashed box with darker red border
    \begin{simpledashbox}{red}{red!70!black}
    \vspace{-0.1cm}
    \noindent \textbf{Tulu-2-DPO-7b ({\color{red} \textbf{Unpreferred}}):} \\
    Architect by day, tech enthusiast by night. Constantly exploring the intersection of design and innovation. Passionate about creating functional and beautiful spaces, both physical and digital. Let's connect and geek out over the latest tech trends!" \#Architecture \#TechEnthusiast \#DesignGeek
    \end{simpledashbox}
\end{multicols}
\label{emoji example}
\end{promptbox}
\end{figure*}

==> tables/pattern-debias.tex <==
\begin{table*}[htp]
\vspace{-3em}
\centering 
\small
% \setlength{\tabcolsep}{2pt}
% \begin{tabular}{lccccccc} 
% \toprule 
% \multirow{2}{*}{\textbf{Debias Type}} & 
% \multirow{2}{*}{$\lambda_C$} & \multicolumn{2}{c}{\textbf{Win-Rate (\%)}} & \multicolumn{4}{c}{\textbf{Rewardbench Evaluation}} \\
% & & Bold & List & Chat & Chat Hard & Safety & Reasoning  \\
% \midrule 
% None & 0 & 89.0 & 92.5 & 0.97 & 0.72 & 0.82 & 0.88 \\ \hline
% Bold* & 0.1 & 54.5 & - & 0.95 & 0.68 & 0.80 & 0.83 \\
% Bold & 0.1 & 56.0 & - & 0.82 & 0.61 & 0.69 & 0.79 \\
% Bold* & 0.2 & 52.5 & - & 0.94 & 0.68 & 0.77 & 0.84 \\
% Bold & 0.2 & 53.5 & - & 0.76 & 0.58 & 0.65 & 0.73 \\
% Bold* & 0.5 & 53.0 & - & 0.95 & 0.67 & 0.77 & 0.85 \\
% Bold & 0.5 & 53.0 & - & 0.63 & 0.52 & 0.59 & 0.66 \\
% %Bold* & 1.0 & 52.5 & - & 0.91 & 0.63 & 0.74 & 0.81 \\
% %Bold & 1.0 & 52.0 & - & 0.51 & 0.49 & 0.55 & 0.63 \\
% List & 0.1 & - & 57.0 & 0.96 & 0.71 & 0.80 & 0.88 \\
% List & 0.2 & - & 55.0 & 0.88 & 0.65 & 0.72 & 0.81 \\
% %List & 0.5 & - & 53.0 & 0.69 & 0.57 & 0.63 & 0.71 \\
% %List & 1.0 & - & 53.0 & 0.55 & 0.51 & 0.54 & 0.66 \\
% \bottomrule 
% \end{tabular}
\begin{tabular}{lccccccc} 
\toprule 
\multirow{2}{*}{\textbf{Debias Type}} & 
\multirow{2}{*}{\textbf{Coefficient}} & \multicolumn{2}{c}{\textbf{Win-Rate (\%)}} & \multicolumn{4}{c}{\textbf{Evaluation(Filtered)}} \\
& & Bold & List & Chat & Chat Hard & Safety & Reasoning  \\
\midrule 
None & - & 89.0 & 92.5 & 98.3 & 71.4 & 83.1 & 85.1 \\ \midrule
Bold* & 0.1 & 54.5 & - & 98.0 & 72.5 & 83.3 & 88.6 \\
Bold & 0.1 & 56.0 & - & 84.2 & 63.3 & 75.8 & 81.0 \\
Bold* & 0.2 & 52.5 & - & 97.5 & 71.1 & 83.0 & 87.3 \\
Bold & 0.2 & 53.5 & - & 81.5 & 60.9 & 70.7 & 77.6 \\
% Bold* & 0.5 & 53.0 & - & 0.95 & 0.67 & 0.77 & 0.85 \\
% Bold & 0.5 & 53.0 & - & 0.63 & 0.52 & 0.59 & 0.66 \\
%Bold* & 1.0 & 52.5 & - & 0.91 & 0.63 & 0.74 & 0.81 \\
%Bold & 1.0 & 52.0 & - & 0.51 & 0.49 & 0.55 & 0.63 \\
List & 0.1 & - & 57.0 & 98.4 & 71.6 & 82.9 & 88.9 \\
List* & 0.1 & - & 54.0 & 98.4 & 72.9 & 83.6 & 89.4 \\
List & 0.2 & - & 55.0 & 92.7 & 67.9 & 76.3 & 84.8 \\
List* & 0.2 & - & 54.0 & 97.5 & 71.3 & 83.0 & 88.6 \\
Bold \& List* & 0.2 & 50.5 & 53.0 & 97.2 & 72.8 & 82.9 & 89.7\\
$\text{Bold \& List}^{\dagger}$ & - & 49.0 & 52.5 & 92.2 & 64.4 & 75.5 & 81.4\\
\bottomrule 
\end{tabular}

\caption{\footnotesize Results of pattern debiasing in reward model training. * indicates reordering and $\dagger$ indicates deleting the response pairs containing responses with patterns.}
\label{tab:debias}
\end{table*}

==> tables/patterns-on-AlpacaEval.tex <==
\begin{table*}[h!]
\vspace{-3em}
\setlength{\tabcolsep}{2pt} \small
\centering
\begin{tabular}{lccccccc} \toprule \textbf{Model} & \textbf{Dataset} & \textbf{Bold (\%)} & \textbf{List (\%)} & \textbf{Exclamation (\%)} & \textbf{Link (\%)} & \textbf{Emoji (\%)} \\
\midrule Llama-3-8B-it & AlpacaEval & 53.63 & 67.50 & 48.13 & 1.00 & 0.38  \\ 
\midrule Gemma-2-9B-it & AlpacaEval & 86.88 & 79.38 & 50.00 & 2.13 & 6.00  \\
\midrule Storm-7B & AlpacaEval & 83.60 & 66.34 & 39.50 & 1.74 & 1.74  \\ 
\midrule Gemma-2-9B-SimPO & AlpacaEval & 90.93 & 76.27 & 31.43 & 0.99 & 4.10 \\ 
\midrule Gemma-2-9B-WPO-HB & AlpacaEval & 96.40 & 81.99 & 43.85 & 0.99 & 8.94 \\ 

\bottomrule \end{tabular}
\caption{We compute the ratio of samples containing specific patterns for the high-ranking models on the AlpacaEval leaderboard. Also see the full table in Table~\ref{tab:policy_model_evaluation_full}. }

\label{tab:policy_model_evaluation}
\end{table*}

==> tables/preference-bias.tex <==
\begin{table*}[t]
\vspace{-3em}
\small
\centering 
% \scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{lcccccccccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Num}} & \multirow{2}{*}{\textbf{Labeller}} & \multirow{2}{*}{\textbf{Type}}  & \multirow{2}{*}{\textbf{Length}} & \multicolumn{6}{c}{\textbf{Ratio of Responses with Pattern (\%)}} \\
&&&&&  \textbf{Bold} & \textbf{List} & \textbf{Emoji} & \textbf{Exclamation} & \textbf{Link} & \textbf{Affirmative} \\
\midrule
\multirow{2}{*}{RLHFlow-Preference} & \multirow{2}{*}{700000} & \multirow{2}{*}{Mixture} &
Preferred & 167.30 & 0.495 & 15.41 & 0.495 & 2.40 & 14.99 & 5.58 \\
&&& Unpreferred & 140.01 & 0.614 & 15.93 & 0.614 & 1.74 & 10.77 & 5.19 \\
\midrule
\multirow{2}{*}{LMSYS-Arena} & \multirow{2}{*}{49865} & \multirow{2}{*}{Human} &
Preferred & 191.64 & 0.073 & 18.52 & 0.073 & 7.61 & 38.84 & 7.30 \\
&&& Unpreferred & 159.77 & 0.616 & 15.77 & 0.616 & 4.54 & 31.67 & 6.45 \\
\midrule
\multirow{2}{*}{AlpacaEval} & \multirow{2}{*}{207687} & \multirow{2}{*}{GPT-4}  &
Preferred & 297.62 & 1.635 & 21.87 & 1.635 & 32.13 & 57.16 & 9.64 \\
&&& Unpreferred & 199.79 & 1.042 & 18.84 & 1.042 & 9.27 & 42.99 & 7.54 \\
\midrule
% \multirow{2}{*}{UltraFeedback\_Binarized} & \multirow{2}{*}{340025} & \multirow{2}{*}{GPT-4} &
% Preferred & 202.60 & 1.045 & 23.39 & 1.045 & 3.25 & 34.20 & 11.81 \\
% &&& Unpreferred & 155.48 & 1.048 & 23.96 & 1.048 & 2.00 & 23.34 & 10.92 \\
% \midrule
\multirow{2}{*}{\href{https://huggingface.co/datasets/HuggingFaceH4/ultrafeedback_binarized}{Ultrafeedback-binarized}} & \multirow{2}{*}{61135} & \multirow{2}{*}{GPT-4} &
Preferred & 198.34 & 1.081 & 22.50 & 1.081 & 3.15 & 34.52 & 10.94 \\
&&& Unpreferred & 175.48 & 1.004 & 23.96 & 1.004 & 2.62 & 27.88 & 11.72 \\
\bottomrule
\end{tabular}
\caption{\footnotesize Statistics summarization of different preference datasets. We compute the proportions of samples with certain formats in both the preferred and unpreferred responses. For length, we compute the number of words of the responses. 
% The UltraFeedback\_Binarized dataset is generated by randomly selecting two responses with the same instruction from the UltraFeedback dataset and assigning a preference based on their scores.
}
\label{tab:dataset_stat}
\end{table*}

==> tables/preference_summary.tex <==
\begin{table*}[h!]
\vspace{-3em}
\setlength{\tabcolsep}{2pt} \small
\centering
\begin{tabular}{lccccccc} \toprule \textbf{Model} & \textbf{Dataset} & \textbf{Bold (\%)} & \textbf{List (\%)} & \textbf{Exclamation (\%)} & \textbf{Link (\%)} & \textbf{Emoji (\%)} \\
\midrule Llama-3-8B-it & AlpacaEval & 53.63 & 67.50 & 48.13 & 1.00 & 0.38  \\ 
\midrule Gemma-2-9B-it & AlpacaEval & 86.88 & 79.38 & 50.00 & 2.13 & 6.00  \\
\midrule Storm-7B & AlpacaEval & 83.60 & 66.34 & 39.50 & 1.74 & 1.74  \\ 
\midrule Gemma-2-9B-SimPO & AlpacaEval & 90.93 & 76.27 & 31.43 & 0.99 & 4.10 \\ 
\midrule Gemma-2-9B-WPO-HB & AlpacaEval & 96.40 & 81.99 & 43.85 & 0.99 & 8.94 \\ 

\bottomrule \end{tabular}
\caption{We compute the ratio of samples containing specific patterns for the high-ranking models on the AlpacaEval leaderboard. Also see the full table in Table~\ref{tab:policy_model_evaluation_full}. }

\label{tab:policy_model_evaluation}
\end{table*}

==> tables/specific_patterns.tex <==
\begin{table}[htp]
    \centering
    \small
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{cccccc}
    \toprule
    Pattern& Type  & Chat & Chat-Hard & Safety & Reasoning\\ \midrule
    \multirow{2}{*}{Bold} & Preferred & 1.44 & 0.11 & 0.47 & 0.05\\
    & Unpreferred & 0.00 & 0.13 & 0.04 & 0.00 \\ \midrule
 \multirow{2}{*}{List} & Preferred & 3.69 & 0.89 & 3.68 & 0.16\\
    & Unpreferred & 0.64 & 2.67 & 8.36 & 0.31 \\ \bottomrule    \end{tabular}
    \caption{The ratio (\%) of samples containing specific pattern and its competitor does not.}
    \label{tab:rewardbench}
\end{table}
